Differential geometric bifurcation problems in pde2path -- algorithms and tutorial examples

We describe how some differential geometric bifurcation problems can be treated with the MATLAB continuation and bifurcation toolbox pde2path. The basic setup consists in solving the PDEs for the normal displacement of an immersed surface $X\subset\mathbb{R}^3$ and subsequent update of $X$ in each continuation step, combined with bifurcation detection and localization, followed by possible branch switching. Examples treated include some minimal surfaces such as Enneper's surface and a Schwarz-P-family, some non-zero constant mean curvature surfaces such as liquid bridges and nodoids, and some 4th order biomembrane models. In all of these we find interesting symmetry breaking bifurcations. Some of these are (semi)analytically known and thus are used as benchmarks.

==> hcaf6.tex <==
\begin{figure}[ht]
\centering 
\btab{l}{%{\sm (a)}{\sm (a)}\\[0mm]
\ig[width=56mm]{hca/bdE}
\hs{-0mm}\rb{23mm}{\btab{ll}{
\ig[height=28mm]{hca/c0b-20}
&\hs{-0mm}\ig[height=26mm]{hca/c0b-40}\\
\hs{-0mm}\ig[height=30mm]{hca/c0b-65}
&\hs{-0mm}\ig[height=30mm]{hca/c0-15}}}\\[-3mm]
\hs{-0mm}\ig[width=59mm]{hca/c1q-15}
\hs{-1mm}\ig[width=59mm]{hca/c2q-16}
\hs{1mm}\ig[width=59mm]{hca/c3q-12}
}
\vs{-4mm}
\caption{{\small Results for \reff{HCd} from {\tt cmds2.m}. 
(a) Continuation in $c_0$ from {\tt b/pt15}, $(\al,\lam_1,b)=(1,0.25,-3.8)$, 
starting from $c_0=0.5$. Blue stable after fold, makes sense and fun!!! 
All symmetric in $(c_0,z)\mapsto -(c_0,z)$. 
\label{hcaf2}}}
\end{figure}

==> hcaf6b.tex <==
\begin{figure}[ht]
\centering 
\btab{l}{{\sm (a)}\\[-2mm]
\hs{-2mm}\ig[width=56mm]{hca/bdE2b}
\rb{40mm}{\btab{ll}{
\hs{-5mm}\ig[height=28mm]{hca/c01b-55}
&\hs{-5mm}\ig[height=28mm]{hca/c01b-2-9}\\[-3mm]
\hs{-5mm}\ig[height=56mm]{hca/c01b-1-16}
&\hs{-5mm}\rb{0mm}{\ig[height=56mm]{hca/c01b-1-24}}}}\\[-4mm]
{\sm (b)}\\
\hs{-2mm}\ig[width=44mm]{hca/bdE4}
\hs{-0mm}\rb{2mm}{\ig[width=44mm]{hca/c1b-1-19}
\hs{-1mm}\ig[width=44mm]{hca/c1b-2-18}
\hs{1mm}\ig[width=44mm]{hca/c1b-2-1-10}}
}
\vs{-4mm}
\caption{{\small %Further results for \reff{HCd} from {\tt cmds1.m}. 
(a) Continuation in $c_0$ from {\tt bb/pt20}, $(\al,\lam_1,b)=(1,0.25,-3.4)$, 
starting from $c_0=0.5$, branches {\tt c01b} (black, to decreasing $c_0$) and 
{\tt c01} (grey, to increasing $c_0$}). There are now two BPs on the unstable 
part of {\tt c01b} for $c_0<0$, and the symmetric BPs for $c_0>0$. 
The blue branch {\tt c01b-1q} (blue) has azimuthal wave number $m=1$ 
and is stable after its fold. %, e.g., {\tt c01b-1q/pt16}. 
The red branch {\tt c01b-2q} has $m=2$ 
and connects to the symmetric BP at $c_0>0$. 
(b) Similarly starting at {\tt bb/pt24} with $b\approx -4$; zoom of BD 
near upper left fold of the branch {\tt c02b} (black) 
similar to {\tt c01b} from (a). Now there is a secondary BP on the 
$m=2$ branch {\tt c02b-2q} (red), giving the magenta branch {\tt c02b-2q-1}. 
\label{hcaf2}}
\end{figure}

==> hcaf7.tex <==
\begin{figure}[h]
\centering 
\hs{-4mm}\ig[width=44mm]{hca/bdE4}
\hs{-0mm}\rb{5mm}{\ig[width=44mm]{hca/c1b-1-19}
\hs{-1mm}\ig[width=44mm]{hca/c1b-2-18}
\hs{1mm}\ig[width=44mm]{hca/c1b-2-1-10}}
\caption{{\small Initial results for \reff{HCd} from {\tt cmds1.m}: 
\label{hcaf2a}}}
\end{figure}

==> hcaf8.tex <==
\begin{figure}[h]
\centering 
\btab{l}{{\sm (a)}\\[-5mm]
\hs{-2mm}\ig[width=38mm]{hca2/bdb2}
\rb{25mm}{\btab{l}{\ig[width=45mm]{hca2/b1-0}
\ig[width=45mm]{hca2/b1-10}
\ig[width=45mm]{hca2/b1-25}\\
\ig[width=45mm]{hca2/b3-9}
\ig[width=45mm]{hca2/b3-14}}}\\
{\sm (b)}\\
\hs{-2mm}\ig[width=38mm]{hca2/bdl}
\ig[width=45mm]{hca2/l1-7}
\ig[width=45mm]{hca2/l3-11}
\ig[width=45mm]{hca2/l3-14}
}

\vs{-4mm}
\caption{{\small cont in $b$ and $\lam_1$
\label{hcaf8}}}
\end{figure}

==> hcylf10b.tex <==
\begin{figure}[H]
\centering 
\btab{ll}{{\sm (a)}&{\sm (b)}\\[-0mm]
\hs{-2mm}\ig[height=42mm,width=24mm]{h8/c0b3}
\hs{-0mm}\ig[height=42mm,width=24mm]{h8/delb3}
&\hs{-6mm}\ig[height=42mm]{h8/010}\hs{-6mm}\ig[height=42mm]{h8/025}
\hs{-8mm}\ig[height=42mm]{h8/026}
}
\\
\btab{l}{{\sm (c)}\\
\hs{-2mm}\ig[height=50mm]{h8/33}\hs{1mm}\ig[height=50mm]{h8/46}
\hs{-0mm}\ig[height=50mm]{h8/46z}\hs{2mm}\ig[height=50mm]{h8/c1-5}}
\vs{-2mm}
\caption{{\small $(\al,\eps)=(1,1/4)$, continuation of Helfrich cylinder 
to $c_0>0$ (blue branch {\tt c0}, {\tt c0r} after mesh refinement), 
with bifurcation to {\tt c1r} (red). Different colormap in samples 
for better visibility of mesh. On {\tt c0}, results after {\tt pt33} 
become somewhat mesh--dependent, but our experiments suggest that the 
branch connects to two hemispheres at $c_0=1/2$ (with {\tt c0r/pt46} 
shortly before that connection). 
\label{hf3b}}}
\end{figure}

==> hcylf10b2.tex <==
\begin{figure}[ht]
\centering 
\btab{ll}{{\sm (a)}&{\sm (b)}\\[-0mm]
\hs{-2mm}\ig[height=50mm]{h8/c0b4}
\hs{-0mm}\ig[height=50mm]{h8/delb4}
&\hs{-6mm}\ig[height=52mm]{h8/010}\hs{-6mm}\ig[height=52mm]{h8/026}
%\hs{-8mm}\ig[height=42mm]{h8/026}
}
\\
\btab{l}{{\sm (c)}\\
\hs{-2mm}\ig[height=50mm]{h8/33}\hs{1mm}\ig[height=50mm]{h8/46}
\hs{-0mm}\ig[height=50mm]{h8/46z}\hs{2mm}\ig[height=50mm]{h8/c1-5}}
\vs{-2mm}
\caption{{\small $(\al,\eps)=(1,1/4)$, continuation of Helfrich cylinder 
to $c_0>0$ (blue branch {\tt c0}, {\tt c0r} after mesh refinement), 
with bifurcation to {\tt c1r} (red). Different colormap (yellow$>$pink) 
in samples 
for better visibility of mesh. On {\tt c0}, results after {\tt pt33} 
become somewhat mesh--dependent, but our experiments suggest that the 
branch connects to two hemispheres at $c_0=1/2$ (with {\tt c0r/pt46} 
shortly before that connection). 
\label{hf3b}}}
\end{figure}

==> hcylf20.tex <==
\begin{figure}[h]
\centering 
\btab{l}{{\sm (a)}\hs{140mm}{\sm (b)}
\\[-0mm]
\hs{-2mm}\rb{0mm}{\ig[height=35mm]{hcp2/bdsEa}
%\ig[height=40mm]{hcp2/bdsEa}
}
\hs{-0mm}\ig[height=32mm]{hcp2/c0b-10}
\hs{-0mm}\ig[height=32mm]{hcp2/c0b-30}
\ig[height=35mm]{hcp2/bdsEb}
\\
{\sm (c)}\\
%\ig[height=40mm]{hcp2/bdsEb}
\rb{5mm}{\hs{-0mm}\ig[height=31mm]{hcp2/c0-15}
\hs{-0mm}\ig[height=31mm]{hcp2/c0-20}
\hs{-0mm}\ig[height=31mm]{hcp2/c0-30}
\hs{-0mm}\ig[height=31mm]{hcp2/c1-5}}

}
\vs{-4mm}
\caption{{\small Results for \reff{HCd} from {\tt cmds4.m}, $\al=0.6$.
pearling. 
\label{hf20}}}
\end{figure}

==> hcylf21.tex <==
\begin{figure}[h]
\centering 
\btab{l}{
\hs{-0mm}\ig[height=40mm]{hcp2/bdbE}
\hs{-0mm}\ig[height=37mm]{hcp2/bc0b-5}
\hs{-0mm}\ig[height=37mm]{hcp2/bc0-20}
\hs{-0mm}\ig[height=37mm]{hcp2/bc0-51}
\hs{-0mm}\ig[height=37mm]{hcp2/bc1-15}

}
\vs{-4mm}
\caption{{\small Results for \reff{HCd} from {\tt cmds3.m}, $\al=1.4$.
\label{hf21}}}
\end{figure}

==> hcylf2b.tex <==
\begin{figure}[H]
\centering
\btab{l}{{\sm (a)}\hs{50mm}{\sm (b)}\hs{40mm}{\sm (c)}\hs{40mm}{\sm (d)}\\
\ig[height=48mm]{h5/l1bd}\ig[height=46mm]{h5/l0b-5}
\hs{-1mm}\ig[height=48mm]{h5/l0-36}
\hs{-4mm}\ig[height=48mm]{h5/l1q-8}\\[-2mm]
{\sm (e)}\hs{50mm}{\sm (f)}\\
\hs{0mm}\ig[height=52mm]{h5/l1qr-32z}\hs{-4mm}\ig[height=50mm]{h5/l2qr-36}
\hs{-10mm}\ig[height=50mm]{h5/l3qr-30}\hs{-2mm}\ig[height=50mm]{h5/l4qr-34}\\
\\[-6mm]
{\sm (g)}\hs{50mm}{\sm (h)}\hs{50mm}{\sm (i)}\\
\ig[height=57mm]{h6/lbd2b2}
\hs{-3mm}\ig[height=54mm]{h6/l0-70}
\hs{-2mm}\rb{5mm}{\ig[height=40mm]{h6/l1-25}}
\hs{-4mm}\ig[height=57mm]{h6/l1-40}
}
\vs{-4mm}
\caption{{\small Results from {\tt cmds2.m} and {\tt cmds2b.m}. 
Continuation in $\lam_1$ at $c_0=0.7$ (a-f), and at 
$c_0=0$ (g,h). In (a): 
axisymmetric branch  {\tt l0b} (dark blue, sample in (b)), 
{\tt l0} (blue, sample in (c))), and 
four bifurcating branches, {\tt l1} (red, refined to {\tt l1qr}, 
samples in (d) and (e), with zoom), 
{\tt l2} (magenta), {\tt l3} (orange), {\tt l4} (green), samples in (f). 
The kinks of {\tt l1}--{\tt l4} 
are due to adapative mesh refinement every 5th step (after pt10), 
from ${\tt np}=2700$ to ${\tt np}\approx 3600$ at the end of each 
branch. In (g) ($c_0=0$) we use the same color code for the branches 
as in (a), 
and have, e.g., {\tt np}=4400 at {\tt 0l1qr/pt40} (i), 
i.e.~{\tt nu}=2{\tt np}=8800 DoF. 
  \label{hf2}}}
\end{figure}

==> hs.tex <==
\section{Spheres, hemispheres, and VPMCF}\label{hssec0}
\subsection{Spheres}\label{spsec}
The demo {\tt spheres}, containing only the (somewhat minimal) files 
{\tt sG.m}, {\tt getM.m}, {\tt sphereinit.m}, and 
{\tt cmds1.m}, 
is mostly meant to illustrate volume preserving mean curvature 
flow (VPMCF) near  spheres, see Fig.~\ref{sf1}.%
\footnote{Additionally, it contains {\tt convtest.m} for convergence 
tests, see Fig.~\ref{nf1}.} 
We refer to {\tt sphereinit.m} and 
{\tt cmds1.m} for comments (and to {\tt geomflow.m} and 
{\tt vpmcff.m} from {\tt libs/Xcont} for the VPMCF) 
and here only note: 
\input{sf1}
\bcen 
\item The comparison between $rA/3$ and $V$ in (a) shows 
a very small error which indicates that the solutions can be safely regarded 
as spheres. 
\item For convex closed initial $X$ (meaning that $X=\pa\Om$ for 
a convex domain $\Om\subset\R^3$), the VPMCF converges to a sphere. 
See also, e.g., \cite{ESi98} for theoretical background. 
This also holds for ``slightly'' non--convex initial $X$ as 
in Fig.~\ref{sf1}(d).% 
\footnote{In detail, $X(0)$ here is obtained as $X(0)=S_{r_0}+(\sin(\vt)(|x|-{r_0})+\xi)N$, where $\xi=0.2({\tt rand}-0.5)$ with {\tt rand} a \mlab\ 
random variable on each node.} 
\item  
Our (explicit Euler) implementation of the VPMCF does not 
conserve $V$ exactly, but with ``reasonable accuracy'', i.e.: 
Even for quite ``non--spherical'' initial $X(0)$, the error 
$|1-V_\infty/V_0|{<}0.01$, where $V_\infty=\lim_{t\to\infty}V(t)<V_0$ 
in all our tests, i.e., $V_\infty$ is always slightly smaller than 
$V_0$.%
\footnote{This ``volume--accuracy'' of {\tt geomflow} for VPMCF 
depends weakly on the Euler--stepsize {\tt dt}, and more strongly 
on the fineness of the discretization of $X$. This can be checked 
by changing {\tt sw} in {\tt spheres/cmds1.m} for initializing $X$.} 
\item During continuation, the position of {\tt X} is not fixed, i.e., 
we have the threefold (approximate) 
translational symmetry in $x,y,z$, and hence always a three-dimensional 
(approximate) kernel. This could be removed by suitable trannslational 
PCs (see the demo {\tt halfspheres}). However, the approximate 
kernel is not a problem for the continuation here (since 
in the Newton loops the right hand sides are orthogonal to this kernel), 
and since we are mostly interested in the VPMCF we refrain from 
these PCs here to keep the demo as sleek and simple as possible. 
\ecen

\subsection{Hemispheres}\label{hssec}
In the demo {\tt hemispheres} we continue  in volume $V$ hemispheres $X$ 
sitting on the $z=0$--plane, i.e., 
\huga{\label{sNBC}
\text{$\pa_r X_3=0$ where $r=\sqrt{x^2+y^2}$,}
}  
and test VPMCF for pertubations of such hemispheres, see Fig.~\ref{sf2}. 
Additionally we use the PCs 
\huga{\label{hspc}
\int_X N_1\dd S=\int_X N_2\dd S=0, \quad X=X_0+uN_0. 
} 
\input{sf2}

\taskip
\begin{table}[ht]\caption{
Files in {\tt pde2path/demos/geomtut/hemispheres}. 
\label{hstab1}}
\centering\vs{-2mm}
{\small 
\begin{tabular}{l|l}%p{0.2\tew}|p{0.82\tew}} 
%file&remarks\\ \hline
{\tt cmds1.m}&continuation in $V$, and VPMCF flow test. \\
{\tt hsinit.m, sGhs.m}&init and rhs\\
{\tt qf2.m, qjac2.m}&PC \reff{hspc}, and derivative \\
{\tt getN.m}&mod of getN, correction at $z=0$\\
{\tt diskpdeo2.m}&mod of (\pdep--)default  {\tt diskpdeo2.m} to have 
a finer mesh at $r=1$. 
\end{tabular}
}
\end{table}
\teskip


Compared to the spheres in \S\ref{spsec} this requires a few more files, 
listed in Table \ref{hstab1}. The PCs \reff{hspc} (and $u$--derivatives) 
are implemented in {\tt qf2, qjac2}, and the rhs $G(u)=H-H_0$ in 
{\tt sGhs} is augmented to $\wt G(u)=H-H_0+s_x N_1+s_y N_2$ 
with multipliers $s_x,s_y$. These stay $\CO(10^{-6})$ during continuation, 
and the only effect of the construction is that 
the now 2D kernel of translational invariance of $\pa_u G$  is removed from 
the linearization of the extended system $(\wt G,q)$. See the end of 
{\tt cmds1.m} for further comments.%
\footnote{In {\tt cmds1.m} we also monitor the ``positions'' $(x_0,y_0)$ 
of $X$ defined as $x_0=\int_X X_1\dd S,\, y_0=\int_X X_2\dd S$. These behave 
as expected, namely: small drifts for continuation without PCs, 
but no drifts for continuation with the PCs \reff{hspc}.} 

The BCs \reff{sNBC} allow movement 
of $\pa X$ in the ``support--plane'' $z=0$, and 
are implemented as %{\tt sGhs} as
$$\text{ {\tt r(idx)=grXz*(X(idx,1).\^{}2+X(idx,2).\^{}2)}($\stackrel!=0$)}$$ 
in {\tt sGhs}, where as usual {\tt idx} are the boundary indizes, and  
{\tt grXz} is the $z$--derivative (operator) 
on $X$, as before obtained from {\tt grX=grad(X,p.tri)} 
and interpolation to the nodes. This forces the $x,y$--coordinates of 
the points on $X$ directly above the $z=0$ layer to be essentially 
equal to those in the $z=0$ layer, i.e., we obtain a 'cylindrical base' 
for the hemispheres. To mitigate this effect, in {\tt hsinit} we 
initialize with a somewhat specialized mesh over the unit disk $D$ 
with higher density towards $\pa D$, which is then mapped to the 
unit hemisphere via $z=\sqrt{1-x^2-y^2}$. Nevertheless, after continuation 
to larger $V$, which is combined with some mesh--adaptation by area, 
we obtain a slight mismatch between $rA/3$ and $V$, 
see Fig.~\ref{sf2}(a,b), and compare Fig.~\ref{sf1}(b).  

In Fig.~\ref{sf2}(c,d) we give an example of VPMCF from a perturbation 
of {\tt hs1r/pt50}, here of the form $X|_{t=0}=X+0.4(\cos(\vt)(\max(z)-z
+0.1({\rm rand}-0.5))N$, where $\vt$ is the angle in the $z=0$ plane. 
We {\em do not use any BCs}  
in the rhs {\tt vpmcff.m}. Instead, we use the correction 
\huga{\label{hsNc}
\text{{\tt N(p.idx,3)=0; N=normalizerow(N)}} 
}
in {\tt getN.m}.
Without \reff{hsNc}, the {\em continuation} of hemispheres 
essentially works as before, 
but the solutions of the VPMCF start to (slowly) lift off the $z=0$ plane, 
and then (quickly) evolve towards a planar $X$ such that also $V\to 0$. 
With \reff{hsNc}, the solutions flow back to hemispheres, 
and $V$ is again conserved up to $0.5\%$, and ``after convergence''  
(e.g., from $X(2)$) we can start continuation again, showing 
consistency. 
%In summary, the demo {\tt hemispheres} 



==> ifig2.tex <==
\begin{figure}[t]
\centering 
\btab{l}{
\btab{ll}{{\sm (a)}&{\sm (b)}\\
\hs{0mm}\ig[width=0.23\tew,height=40mm]{p1/sBD2}
\hs{0mm}\ig[width=0.23\tew]{p1/s5}\ig[width=0.23\tew]{p1/s45}
&\ig[height=0.3\tew,height=44mm]{p5/e1-36}}\\
\btab{lll}{{\sm (c)}&{\sm (d)}&{\sm (e)}\\
\hs{0mm}\rb{6mm}{\ig[width=0.33\tew]{nopi1/n1-6}}
%&\ig[width=0.32\tew]{mpi3/ln2a-10b}
&\rb{10mm}{\ig[width=0.24\tew]{tps/p-1}}&
%\rb{10mm}{\ig[width=55mm]{hca2/bc2-0}}
\rb{5mm}{\ig[height=50mm]{hca/c01b-1-16}}
}
}
\vs{-8mm}
\caption{{\small Preview of solutions (solution branches) we compute. 
(a) $H$ over $V$ for spherical caps, 
and sample solutions, \S\ref{scsec}. The colors indicate $u$ in the 
last continuation step, yellow$>$blue, and thus besides giving visual structure 
to $X$ indicate the ``direction'' of the continuation. 
$H$ is negative since here $N$ is the outer 
normal. (b) Enneper minimal surface (a bounded part, with the boundary 
shown in red), \S\ref{ensec}. 
(c) A liquid bridge between two circles, with excess volume and 
hence after a symmetry breaking bifurcation, \S\ref{snsec}. 
(d) A Schwarz P surface, \S\ref{SPsec}. 
(e) A Helfrich--type biomembrane cap after a symmetry breaking bifurcation. 
Samples (b)--(e) are each 
again from branches of solutions of the respective 
problems, see Figures \ref{ef1}, \ref{nodf0}, \ref{tpsf1} and \ref{hcaf2}
for the bifurcation diagrams.
\label{f1}}}
\end{figure}

==> scfe2b.tex <==
\begin{figure}[ht] 
\centering
\btab{lll}{{\sm (a)}&{\sm (b)}&{\sm (c)}\\
\hs{-2mm}\rb{2mm}{\ig[height=0.29\tew]{p4/l2e2b}}
&\hs{-2mm}\rb{2mm}{\ig[height=0.29\tew]{p4/mq}}
&\hs{-5mm}\ig[height=0.29\tew]{p4/25}
\hs{0mm}\ig[height=0.29\tew]{p4/27}
%\hs{-3mm}\ig[height=0.33\tew]{p4/132}
}
\vs{-4mm}
\caption{{\small Results from {\tt spcap1/cmds2.m}. (a) 
Error $e(X):=\|H-H(V)\|_2/|H(V)|$ for refinement each 15th step 
({\tt capr1}, black) (starting at step 10), 
when $e(X)>{\tt p.nc.errtol}=0.05$, 
using {\tt p.fuha.ufu=@refufu} ({\tt capr3}, red), and when 
$\max(A)>0.3$ using  {\tt p.fuha.ufu=@refufumaxA} with $\sig=0.3$ 
({\tt capr4}, magenta). At $V=200$, $n_p=1452$ on {\tt capr1}, 
$n_p=1486$ on {\tt capr3}, and $n_p=636$ on {\tt capr4}. 
(b) Mesh distortion $\delm=\max(h/r)$ (edge-length over in--radius). 
(c) Illustration of meshes before/after refinement at pt25;  plots cropped 
at $y=0$ for better visibility of the meshes, and the boundary 
at $z=0$ marked in red. 
\label{spcf1c}}}
\end{figure}
